Learning Deep Optimal Embeddings with Sinkhorn Divergences

Deep Metric Learning algorithms aim to learn an efficient embedding space to preserve the similarity relationships among the input data. Whilst these algorithms have achieved significant performance gains across a wide plethora of tasks, they have also failed to consider and increase comprehensive similarity constraints; thus learning a sub-optimal metric in the embedding space. Moreover, up until now; there have been few studies with respect to their performance in the presence of noisy labels. Here, we address the concern of learning a discriminative deep embedding space by designing a novel, yet effective Deep Class-wise Discrepancy Loss (DCDL) function that segregates the underlying similarity distributions (thus introducing class-wise discrepancy) of the embedding points between each and every class. Our empirical results across three standard image classification datasets and two fine-grained image recognition datasets in the presence and absence of noise clearly demonstrate the need for incorporating such class-wise similarity relationships along with traditional algorithms while learning a discriminative embedding space.

==> SOUMAVA-FILES/paper_abstract.tex <==
\begin{abstract}
Deep Metric Learning algorithms aim to learn an efficient embedding space to preserve the similarity relationships among the input data. Whilst these algorithms have achieved significant performance gains across a wide plethora of tasks, they have also failed to consider, and increase, comprehensive similarity constraints, thus learning a sub-optimal metric in the embedding space. Moreover, up until now; there have been few studies with respect to their performance in the presence of noisy labels. Here, we address the concern of learning a discriminative deep embedding space by designing a novel, yet effective Deep Class-wise Discrepancy Loss (DCDL) function that segregates the underlying similarity distributions (thus introducing class-wise discrepancy) of the embedding points between each and every class. Our empirical results across three standard image classification datasets and two fine-grained image recognition datasets in the \textbf{presence} and \textbf{absence} of noise clearly demonstrate the need for incorporating such class-wise similarity relationships along with traditional algorithms while learning a discriminative embedding space. 
% \keywords{}
\end{abstract}

\begin{IEEEImpStatement}
Existing metric learning algorithms fail to consider class-wise similarity and dissimilarity relations, thereby failing to learn an optimal embedding space. Here we have proposed a novel algorithm called Deep Class-wise Discrepancy Loss (DCDL), which takes into account such class-wise relationships in terms of probability distributions and aims to separate them in the embedding space using optimal transport based Maximum Mean Discrepancy and Wasserstein Distance. Through rigorous experiments across several experimental setups and five datasets, we have shown that DCDL is able to learn a superior embedding space against various baseline metric learning algorithms. The results obtained clearly demonstrate that one needs to separate such class-wise distributions to further improve the discriminative ability of the embedding space. DCDL has also shown to outperform the baseline algorithms even in the presence of noisy labels, thereby being robust to handle the ill effects of noise so as to simultaneously increase and decrease the inter-class and intra-class variances in the learnt embedding space.
\end{IEEEImpStatement}


\begin{IEEEkeywords}
Deep Metric Learning, Noisy Labels, Optimal Transport, Sinkhorn Divergences.
\end{IEEEkeywords}


==> SOUMAVA-FILES/paper_simple_exps_with_XE.tex <==
\section{Experiments with Cross Entropy Loss:}

In this section, we examine the compatibility of adding the conventional cross entropy loss to the training loss $\mathrm{L_{Train}}$ (Eqn.~(\textcolor{red}{5}) of the main text)
%~\eqref{eqn:train_loss_final}) 
used for $\mathrm{DCDL}$. Thus, our new loss is defined as follows:
\begin{equation}
\label{eqn:train_xent}
    \mathrm{L_{Train}^{xent}} = \mathrm{L_{Train}} + \lambda_{\mathrm{xent}}~\mathrm{L_{xent}}.
\end{equation}



\begin{table}[!h]
\centering
\caption{Experimental results while training with $\mathrm{L_{Train}^{xent}}$ in the \textbf{clean} labels setting. %We report the test classification accuracy (\%) here.
}
\label{tab:res_xent_clean}
\vspace{0.2cm}
\scalebox{1.0}{
    \begin{tabular}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}c|c|c!{\vrule width 1.5pt}}%!{\vrule width 1.5pt}}
    \Xhline{2\arrayrulewidth}
    \backslashbox{Method}{Dataset} & C-10 & C-100 & S-10
    \\ \Xhline{2\arrayrulewidth}
    $\mathrm{L_{xent}}$ &  86.3 & 70.9 & 65.7
    \\ \Xhline{2\arrayrulewidth}
    $\mathrm{L_{Trip}}~+~\mathrm{L_{xent}}$ & 87.2 & 71.2 & 67.9 \\
    $\mathrm{L_{Trip}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$ & 87.8 & 72.4 & 69.2 \\
    $\mathrm{L_{Trip}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$ & 87.9  & 72.1 & 68.8 \\
    \Xhline{2\arrayrulewidth}
    $\mathrm{L_{NP}}~+~\mathrm{L_{xent}}$& 87.3 & 72.1 & 67.7 \\
    $\mathrm{L_{NP}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$ & 87.2 & 71.9 & 68.2 \\
    $\mathrm{L_{NP}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$ & 89.5 & 72.7 & 67.9
    \\ \Xhline{2\arrayrulewidth}
    
    $\mathrm{L_{Ang}}~+~\mathrm{L_{xent}}$ & 87.1 & 71.5 & 68.2 \\
    $\mathrm{L_{Ang}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$ & 87.6 & 72.0 & 68.9 \\
    $\mathrm{L_{Ang}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$ & 87.9 & 71.8 & 68.5
    \\ 
    \Xhline{2\arrayrulewidth}
    \end{tabular}}
\end{table}

\begin{table}[!b]
\centering
\caption{Experimental results while training with $\mathrm{L_{Train}^{xent}}$ in the \textbf{symmetric} noisy labels setting. %The results reported here denote the classification accuracy (\%) on the test set.
}
\vspace{0.2cm}
\label{tab:res_xent_sym}
\scalebox{0.87}{
\begin{tabular}{c!{\vrule width 1.5pt}c|c|c||c|c|c!{\vrule width 1.5pt}}
\cline{2-7}
 & \multicolumn{3}{c||}{$\delta$=$0.1$} & \multicolumn{3}{c!{\vrule width 1.5pt}}{$\delta$=$0.3$} 
\\ \Xhline{3\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{\backslashbox{Method}{Dataset}}  & \multicolumn{1}{c|}{C-10} & \multicolumn{1}{c|}{C-100} & \multicolumn{1}{c||}{S-10} & \multicolumn{1}{c|}{C-10} & \multicolumn{1}{c|}{C-100} & \multicolumn{1}{c!{\vrule width 1.5pt}}{S-10} 
\\ \Xhline{2\arrayrulewidth}
% $\lambda_{\mathrm{xent}}$ & 1.0 & 1.0 & 1.0 & 1.0 & .0 & 1.0 
% \\ \Xhline{2\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{xent}}$}  & 81.4 &  64.3 & 60.8 & 76.1 & 55.1 & 51.1
\\ \Xhline{2\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Trip}}~+~\mathrm{L_{xent}}$} & 83.1 & 66.5 & 62.8 & 77.1 & 58.2 & 52.1\\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Trip}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$} & 83.0 & 66.3 & 63.1 & 78.2 & 58.7 & 51.9 \\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Trip}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$} & 83.5 & 67.1 & 63.9 & 78.9 & 59.0 & 52.9 \\ \Xhline{2\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{NP}}~+~\mathrm{L_{xent}}$} & 83.2 & 65.8 & 63.6 & 77.5 & 58.8 & 53.4 \\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{NP}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$} & 83.7 & 66.2 & 63.9 & 78.9 & 60.1 & 54.1\\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{NP}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$} & 83.5 & 66.9 & 64.7 & 79.8 & 59.8 & 55.2
\\ \Xhline{2\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Ang}}~+~\mathrm{L_{xent}}$} & 83.2 & 66.3 & 63.4 & 77.9 & 56.6 & 52.8\\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Ang}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$} & 83.6 & 66.1 & 64.5 & 78.6 & 57.7 & 53.2 \\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Ang}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$} & 83.7 & 64.7 & 64.6 & 78.9& 57.5 & 54.1
\\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\end{table}


We have fixed the value of $\lambda_{\mathrm{xent}}$ to $1.0$ in all our experiments. The results are shown in Table~\ref{tab:res_xent_clean},~\ref{tab:res_xent_sym} and~\ref{tab:res_xent_asym} in the clean, symmetric-noisy and asymmetric-noisy labels settings respectively. As observed, and to no surprise, training our models with $\mathrm{L_{Train}^{xent}}$ leads to a significant overall improvement in terms of classification accuracy across all the datasets and experimental settings. Having said that, $\mathrm{L}^{\mathcal{W}}$ still outperforms $\mathrm{L}^{\mathrm{L}}$ in most of the settings except a few, in the presence/absence of noise. To some degree,~$\mathrm{L_{xent}}$ is a partial global loss as it aims to find class-separating sub-spaces in the output (or embedding) space in order to increase the inter-class distances between the embedded points. However, it fails to guarantee that the intra-class distances are reduced within these hyper-planes. With the addition of $\mathrm{L_{Local}}$ such intra-class distances are reduced to some extent; but this too fails to ensure that the class-separating sub-spaces are also distant from one other. Further addition of the discrepancy loss in terms of $\mathrm{L}^{\varphi}$ leads to an increase in the separation between the class-separating sub-spaces due to the disparity induced between the distributions of class-wise embeddings for every class. This indeed demonstrates the need and the ability of $\mathrm{L}^{\varphi}$ to learn discriminant embeddings even in the presence of a partially global cross entropy loss. We also evaluate the $\mathrm{DCDL}$ method on the widely used fine-grained image datasets  \textbf{(a) Caltech-UCSD Birds} (CUBS-$200$-$2011$)~\citep{CUB200_DB} and \textbf{(b) Stanford Cars} dataset (CARS$196$)~\citep{CARS196_DB}. More details are provided in supplementary material.


\begin{table}[t]
\centering
\caption{Experimental results while training with $\mathrm{L_{Train}^{xent}}$ in the \textbf{asymmetric} noisy labels setting. %The test accuracies (\%) is reported here.
}
\label{tab:res_xent_asym}
\vspace{0.2cm}
\scalebox{1.1}{
\begin{tabular}{c!{\vrule width 1.5pt}c|c||c|c!{\vrule width 1.5pt}}
\cline{2-5}
 & \multicolumn{2}{c||}{$\delta$=$0.1$} & \multicolumn{2}{c!{\vrule width 1.5pt}}{$\delta$=$0.2$} 
 
\\ \Xhline{3\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{\backslashbox{Method}{Dataset}} & \multicolumn{1}{c|}{C-10} &  \multicolumn{1}{c||}{S-10} & \multicolumn{1}{c|}{C-10} & \multicolumn{1}{c!{\vrule width 1.5pt}}{S-10} 
\\ \Xhline{2\arrayrulewidth}
% $\lambda_{\mathrm{xent}}$ & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 
% \\ \Xhline{2\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{xent}}$} & 83.8 & 63.9 & 80.7  & 61.4
\\ \Xhline{2\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Trip}}~+~\mathrm{L_{xent}}$} & 84.1 & 65.1 & 80.9 & 62.7\\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Trip}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$} & 84.6 & 65.8 & 81.5 & 64.1 \\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Trip}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$} & 84.3 & 66.4 & 82.3 & 63.8\\ \Xhline{2\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{NP}}~+~\mathrm{L_{xent}}$} & 84.4 & 64.9 & 81.9 & 63.1 \\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{NP}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$} & 84.8 & 66.1 & 82.6 & 63.7 \\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{NP}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$} & 84.2 & 65.8 & 84.1 & 64.0
\\ \Xhline{2\arrayrulewidth}
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Ang}}~+~\mathrm{L_{xent}}$} & 83.9 & 65.1 & 82.4 & 62.4\\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Ang}}~+~\mathrm{L}^{\mathrm{L}}~+~\mathrm{L_{xent}}$} & 84.4 & 65.9 & 82.2 & 64.2 \\
\multicolumn{1}{!{\vrule width 1.5pt}c!{\vrule width 1.5pt}}{$\mathrm{L_{Ang}}~+~\mathrm{L}^{\mathcal{W}}~+~\mathrm{L_{xent}}$} & 84.8 & 66.4 & 82.6 & 64.1
\\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\end{table}
